AraMIP: Extending MIPVU Towards Metaphor Identification in Arabic

Metaphor research has gained increasing attention due to its relevance to linguistic creativity, language use, cognitive processes, and related areas. While many efforts have been devoted to metaphor identification and annotation in English and other languages, Arabic remains under-resourced in this area. In this work, we propose the Arabic Metaphor Identification Procedure (AraMIP), a novel guideline for Arabic metaphor annotation. AraMIP builds on the widely used Metaphor Identification Procedure Vrije Universiteit (MIPVU) framework, incorporating adaptations that accounts for the language-specific properties of Arabic. We distinguish three major types of Arabic figurative language: Isti'ara (metaphor), kinaya (metonymy/indirect expression), and tashbih (simile), and annotate a pilot dataset of 300 sentences (5277 words). Our analysis reveals key challenges specific to Arabic, including morphological complexity, inconsistencies in dictionary sense ordering, and the absence of standardized contextual materials for annotators. This work contributes a first step toward standardized Arabic figurative instances and facilitates the development of larger annotated resources, thereby supporting future research on figurative language in Arabic.

==> guidlines.tex <==
\section{AraMIP}
MIP, MIPVU and adaptation to Arabic

\begin{figure}[h]
\centering
\scalebox{0.60}{
\begin{tikzpicture}[
  boxa/.style={rectangle, rounded corners=4pt, draw=gray, fill=#1, minimum width=10cm, minimum height=0.9cm, align=center, font=\small},
  pill4/.style={rectangle, rounded corners=4pt, draw=gray, fill=#1, minimum width=2.2cm, minimum height=0.7cm, align=center, font=\footnotesize},
  pill3/.style={rectangle, rounded corners=4pt, draw=gray, fill=#1, minimum width=3.0cm, minimum height=0.7cm, align=center, font=\footnotesize},
  node distance=0.4cm
]

%% Stage 1
\node[font=\small\bfseries] (s1title) {Stage 1: Word Level};
\node[boxa=red!15, below=0.2cm of s1title] (s1)
  {\textbf{MIPVU: one code per word}};

%% Row A — 4 narrow pills, place second pill left of center
\node[pill4=red!15, below=0.4cm of s1, xshift=-1.2cm] (b) {MRW direct};
\node[pill4=red!15, left=0.2cm of b]   (a) {MRW indirect};
\node[pill4=red!15, right=0.2cm of b]  (c) {MRW implicit};
\node[pill4=red!15, right=0.2cm of c]  (d) {MFlag};

%% Row B — 3 wider pills centered
\node[pill3=gray!20, below=0.3cm of b, xshift=1.2cm] (e) {MRW negative};
\node[pill3=gray!20, left=0.2cm of e]  (g) {WIDLII};
\node[pill3=gray!20, right=0.2cm of e] (f) {DFMA};

%% Stage 2
\node[font=\small\bfseries, below=1.2cm of e] (s2title)
  {Stage 2: Span Level};
\node[boxa=violet!15, below=0.2cm of s2title] (s2)
  {\textbf{Highlight span $\cdot$ overlapping spans allowed}};

%% 3 rhetorical pills centered
\node[pill3=violet!15, minimum width=3.8cm, below=0.4cm of s2] (kin)
  {Kinaya (literal possible)};
\node[pill3=violet!15, minimum width=3.8cm, left=0.2cm of kin] (isti)
  {Isti\textquoteleft ara (literal impossible)};
\node[pill3=violet!15, minimum width=3.8cm, right=0.2cm of kin] (tash)
  {Tashbih (explicit comparison)};

%% Conventionality
\node[pill3=orange!20, minimum width=9cm, below=0.3cm of s2, yshift=-1.5cm] (conv)
  {Conventionality: (1) (2) (3) (4) (5)};

\end{tikzpicture}
}
\caption{The AraMIP two-stage annotation procedure.}
\label{fig:aramip}
\end{figure}
